PonderV2: Pave the Way for 3D Foundation Model with A Universal Pre-training Paradigm

In contrast to numerous NLP and 2D vision foundational models, learning a 3D foundational model poses considerably greater challenges. This is primarily due to the inherent data variability and diversity of downstream tasks. In this paper, we introduce a novel universal 3D pre-training framework designed to facilitate the acquisition of efficient 3D representation, thereby establishing a pathway to 3D foundational models. Considering that informative 3D features should encode rich geometry and appearance cues that can be utilized to render realistic images, we propose to learn 3D representations by differentiable neural rendering. We train a 3D backbone with a devised volumetric neural renderer by comparing the rendered with the real images. Notably, our approach seamlessly integrates the learned 3D encoder into various downstream tasks. These tasks encompass not only high-level challenges such as 3D detection and segmentation but also low-level objectives like 3D reconstruction and image synthesis, spanning both indoor and outdoor scenarios. Besides, we also illustrate the capability of pre-training a 2D backbone using the proposed methodology, surpassing conventional pre-training methods by a large margin. For the first time, PonderV2 achieves state-of-the-art performance on 11 indoor and outdoor benchmarks, implying its effectiveness. Code and models are available at https://github.com/OpenGVLab/PonderV2.

==> rebuttal.tex <==

\centerline{\textbf{------------------------------------------------------ Responses To Associate Editor ------------------------------------------------------}}


\textbf{Q1: The structure and presentation need to be improved.}

A1: Thanks for your suggestion. All the revisions have been highlighted in the paper in \textcolor{orange}{orange}. 

\textbf{Q2: GCNs are usually slow. The original PointNet works process only about 4000 points. How do the authors manage to scale a GCN to serve as a foundation model backbone?}

A2: In this paper, we utilize \textbf{sparse convolutional networks} as the backbone, which converts irregular points into volumetric representations. These networks are highly efficient, using methods like hash tables to manage data sparsity dynamically. Sparse convolutional networks are widely applied in many state-of-the-art methods for both indoor~\cite{wu2023ppt} and outdoor~\cite{li2022uvtr} scenarios. 

Our network architecture follows a ResNet structure with residual connections, making it easy to scale up the backbone's parameters, similar to traditional 2D convolutional networks. This scalability allows our model to handle large datasets effectively. 

We have tested the speed of SpConv and PointNet encoders in Appendix~\ref{appx:speed}. For convenience, we paste it below and the values are averaged on ScanNet semantic segmentation dataset with a batch size of $3$. The results indicate that sparse convolution is much faster and less memory-consuming than point-based methods even with much more model parameters. This shows its ability to be scaled up and process large datasets.

\setcounter{table}{0}
\begin{table}[!h]\centering
\caption{\textbf{Training speed of different encoders.}}\label{tab:speed2}
\tablestyle{6pt}{1.05}
\begin{tabular}{lccccc}\toprule
Encoder &\#Params &\#Points per Batch &GPU memory &Forward Time \\\cmidrule{1-5}
PointNet &3.53M &$\sim$40K &$\sim$6.0G &$\sim$1.82s \\%\cmidrule{1-5}
PointNet++ &0.97M &$\sim$40K &$\sim$11.0G &$\sim$2.03s \\%\cmidrule{1-5}
PointNet++ &0.97M &$\sim$85K &$\sim$21.0G &$\sim$4.08s \\%\cmidrule{1-5}
SpUNet14 &12.88M &$\sim$85K &$\sim$5.2G &$\sim$0.11s \\%\cmidrule{1-5}
SpUNet18 &23.01M &$\sim$85K &$\sim$5.2G &$\sim$0.11s \\%\cmidrule{1-5}
SpUNet34 &39.16M &$\sim$85K &$\sim$5.5G &$\sim$0.13s \\%\cmidrule{1-5}
SpUNet50 &34.03M &$\sim$85K &$\sim$9.1G &$\sim$0.14s \\%\cmidrule{1-5}
SpUNet101 &73.08M &$\sim$85K &$\sim$9.7G &$\sim$0.17s \\%\cmidrule{1-5}
\bottomrule
\end{tabular}
\end{table}


\textbf{Q3: Rendering signed distance fields is usually slow and a limiting factor. How do the authors manage to make it fast enough to train large models?}

A3: The rendering block acts as the decoder, and after pre-training, we use only the encoder for fine-tuning downstream tasks. To improve efficiency, we render only a subset by randomly selecting 256 pixels per image across a batch of 5 images, enhancing sampling diversity. As tested in Appendix~\ref{appx:speed}, the decoder accounts for approximately $1.7$ seconds per step during pre-training, which is reasonable and affordable. 

\textbf{Q4: The manuscript is lacking a discussion of current training times and how the model would scale to really large datasets.}

A4: Thanks for your suggestion! We have added details on the summary of training times in \tabref{tab:setting_summary}. We've also added pre-training speed analysis in Appendix~\ref{appx:speed}. We can find that our pre-training takes about 2.08 seconds per step which is reasonable and affordable for large-scale datasets.

Due to significant differences in data distribution between indoor and outdoor environments, we pre-train the model separately for each. \tabref{tab:setting_summary} shows the summary of the training details, including data sources, dataset sizes, training times, and the number of steps.
We manage rendering times by optimizing the process for efficiency, as discussed previously, ensuring scalability to large datasets.



\textbf{Q5: The authors are asked to add a table with all the different settings, including the respective task, the active architecture parts, their training data, the loss functions, and the pretraining steps.}

A5: Thanks for your suggestion. The details are listed in \tabref{tab:setting_summary}. For convenience, we paste the table here.
\begin{table*}[!h]
\centering
\caption{Summary of different experimental settings.}\label{tab:setting_summary2}
\vspace{-0.8em}
\tablestyle{1pt}{1.05}
\begin{tabular}{lccccc}\toprule
&\multicolumn{2}{c}{Indoor} &\multicolumn{2}{c}{Outdoor} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
&\secref{sec:rgbd} &\secref{sec:indoor} &\secref{sec:outdoor}& \\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}
Pre-train Datasets &ScanNet~\cite{dai2017scannet} &ScanNet~\cite{dai2017scannet}, S3DIS~\cite{armeni2017joint}, Structured3D~\cite{zheng2020structured3d} & NuScenes~\cite{caesar2020nuscenes}  & \\%\cmidrule{1-4}
Pre-train Data size &$\sim$1500 Scenes &$\sim$5271 Scenes &$\sim$700 scenes & \\%\cmidrule{1-4}
Total Pre-train Epochs &100 &200 &24 & \\%\cmidrule{1-4}
Total Pre-train Time &$\sim$4 days &$\sim$7 days &$\sim$2 days & \\%\cmidrule{1-4}
Input Format &Multi-View RGB-D Images &Scanned Scene Point Clouds &LiDAR Point Clouds / Multi-Camera Images & \\%\cmidrule{1-4}
Pre-trained Architecture &Encoder &Encoder &Encoder + BEV Volume & \\%\cmidrule{1-4}
Loss Functions &\eqref{loss:indoor_rgbd} &\eqref{loss:indoor} &\eqref{loss:render} & \\%\cmidrule{1-4}
\multirow{4}{*}{Downstream Tasks} & Object Detection, & Semantic Segmentation& Object Detection& \\
& Semantic Segmentation, & Instance Segmentation,& Semantic Segmentation& \\
& Scene Reconstruction, & Object Reconstruction,& \etc& \\
& Image Synthesis, \etc& \etc & & \\
\bottomrule
\end{tabular}
\end{table*}


\textbf{Q6: The authors are asked to either provide a clear justification for why this is a foundation model or step towards it or to remove the claims about foundation models entirely (this holds especially for the title, as it is likely to mislead the community).}

A6: Thank you for your feedback. We want to clarify that our intention was not to claim that our pre-trained model is already a foundation model. Instead, our work focuses on demonstrating the pretraining method's effectiveness across multiple tasks and scenarios, showcasing its versatility compared to other methods. This flexibility is a step toward developing a foundation model in the future, but we do not claim to have achieved that yet.

To avoid misunderstanding, we have revised the phrasing in the paper and removed any claims suggesting this is already a foundation model. We have also updated the title to reflect the scope and contributions of our work accurately.

\centerline{\textbf{------------------------------------------------------ Responses To Reviewer 1 ------------------------------------------------------}}

\textbf{Q7: The loss functions described in this paper's pipeline differ from those in the preliminary work.}

A7: Thank you for highlighting this point. In our preliminary work, we included three additional loss terms, as is common in neural reconstruction settings. We have now reintroduced these terms and provided detailed descriptions in \secref{sec:method_indoor_scenario} and Appendix~\ref{appx:loss}. %

\textbf{Q8: In most cases, pre-training in the paper is unsupervised. However, in the experiments in the "Indoor Scene Point Clouds as Inputs" section, the authors use labeled semantics as a supervisory signal during pre-training. How significantly would removing this label supervision affect the model's performance on these benchmarks?}

A8:  Our method benefits from the differentiable nature of the rendering module, allowing us to utilize 2D supervision signals effectively. Even without labeled semantics, we can directly extract knowledge from 2D foundation models by rendering corresponding semantic feature maps. For example, using the ViT-base version of the CLIP visual encoder, the mAP on ScanNet semantic segmentation reaches 76.95, which is very close to the 70.02 mAP achieved with ground truth labels. These results have been added to the paper, further demonstrating the effectiveness and robustness of our approach.


\textbf{Q9: In section 4.2, the authors state, "Considering that although a lightweight decoder reduces the rendering effect, it may boost downstream performance." Is there experimental data to support this? Additionally, in section 5.6, the authors mentioned that the size of the decoder is positively correlated with downstream task performance, which seems contradictory to the above statement}

A9: 
In Section 4.2, we show the results of indoor cases where the volumetric representation is removed during fine-tuning for downstream tasks. The rendering quality in pretraining is highly related to the resolution of the volume representation. \tabref{tab:supp resolution} shows that the accuracy on ScanNet and SUNRGBD remains stable, even with higher volumetric resolutions. Therefore, for efficiency consideration, we use a relatively small single-resolution volume size. We have made the corresponding description more clear in the paper.

On the other hand, pre-trained volumetric features are leveraged for outdoor downstream tasks, where these features are utilized as bird's-eye view (BEV) representations. In these cases, smaller volume resolutions often result in suboptimal performance, as demonstrated in \tabref{tab:decoder_depth}.



\centerline{\textbf{------------------------------------------------------ Responses To Reviewer 2 ------------------------------------------------------}}

\textbf{Q10: Neural rendering and also graph convolutional neural networks are usually slow. What are the training speeds like, and how could sufficient speed be achieved to scale this paradigm to training a foundation model?}

A10: Thanks for your question. Similar to A2, we utilize \textbf{sparse convolutional networks} as the backbone, which converts irregular points into volumetric representations. These networks are highly efficient, using methods like hash tables to manage data sparsity dynamically. Sparse convolutional networks are widely applied in many state-of-the-art methods for both indoor~\cite{wu2023ppt} and outdoor~\cite{li2022uvtr} scenarios. 

Our network architecture follows a ResNet structure with residual connections, making it easy to scale up the backbone's parameters, similar to traditional 2D convolutional networks. This scalability allows our model to handle large datasets effectively. 

We have tested the speed of SpConv and PointNet encoders in Appendix~\ref{appx:speed}. The results indicate that sparse convolution is much faster and less memory-consuming than point-based methods even with much more model parameters. This shows its ability to be scaled up and process large datasets.

\textbf{Q11: A foundation model would be a single model that can extract features in both subdomains. Would it be possible to build a single model using Ponder pretraining/ would Ponder training scale up effectively?}

A11: Thanks for your suggestion. However, it is extremely challenging to use the same set of model parameters to handle both indoor and outdoor data. 
There are significant differences in the distribution characteristics of indoor and outdoor point cloud data. For example, indoor point clouds are often densely reconstructed with consistent point density, while outdoor LiDAR point clouds tend to have an uneven distribution. Additionally, the scale of indoor and outdoor scenes can differ by an order of magnitude. In addition, our intention was not to claim that our pre-trained model is already a foundation model. Instead, our work focuses on demonstrating the pretraining method’s effectiveness across multiple tasks and scenarios, showcasing its versatility compared to other methods. Related description is modified in the latest version.



\textbf{Q12: 3D representations such as RGB point clouds ignore specularities and lighting conditions, all of which require multiple views of the same object. It should be investigated whether the PonderV2-trained network’s features are invariant under these types of changes.}

A12: Thank you for your insightful suggestion. When rendering 3D representations, RGB networks incorporate view direction inputs. This allows the network to encode variations in specularities and lighting conditions effectively, thereby providing a more comprehensive representation of the object from multiple perspectives. Moreover, depth information is generally invariant to changes in lighting and specularities. By incorporating depth supervision, we can mitigate some of the limitations associated with RGB point clouds. Depth supervision ensures that the geometric structure of the object remains consistent across different views, improving the robustness of the representation.


\textbf{Q13: The justification for what is “novel” about the differentiable volume rendering is not articulated. }

A13: Thanks for your suggestion. Related content has been added to the paper.
Unlike previous methods that rely on either contrastive learning or MAE for pretraining, we are the first to explore the advantages of differentiable neural rendering, tailored for learning effective 3D presentation. The proposed pretraining method reaches state-of-the-art performance on many popular benchmarks of both indoor and outdoor and is flexible enough to integrate into various backbones. Neural rendering effectively bridges the gap between the 3D world and 2D representations, allowing us to fully leverage large-scale 2D data to learn effective 3D representation.
As explained in Section 5.2, when our method is applied to training 2D backbones, the learned 3D knowledge proves to be more robust and effective than that obtained through previous representation learning methods.
In this paper, our goal is not to introduce innovations in the rendering method itself but to explore how it can be utilized for learning effective 3D representation.

\textbf{Q14: Fig 3: How is the sparse backbone implemented? What is the loss function?}

A14: 
We used SparseUNet as our sparse backbone. It is a 3D UNet-like architecture with optimized sparse convolutional operations offered by SpConv (\url{https://github.com/traveller59/spconv}). We have offered more implementary details in the paper and Appendix. The loss function of pre-training is detailed in \secref{sec:main_method}.

\textbf{Q15: Page 7, col 2, line 45 introduces the multiresolution feature volume. This is not mentioned in section 3.1 and is not the structure implied in section 3.1 (Page 3, col 2, line 34).}

A15: Thank you for highlighting this point. The multiresolution feature volume is discussed as part of an ablation study. While this technique is common in neural rendering, we found it redundant and unnecessary for representation learning. We aim to demonstrate that a single-resolution volume is both valid and efficient. We have modified related descriptions to make them more clear.


\textbf{Q16: Page 7, col 2, line 12: “Following the pre-training phase, we discard the rendering decoder and load the encoder backbone’s weights for use in downstream tasks”. This point is critical and should be emphasized earlier in the text.}

A16: Thanks for your suggestion, we have modified the paper. 


\textbf{Q17: The inclusion of the words “Foundation Model” in the title, first line, and elsewhere in the manuscript can make a reader expect that a foundation model will be produced.}

A17: Thank you for your suggestion. We want to clarify that our intention was not to claim our pre-trained model is already a foundation model. Our work focuses on demonstrating the pretraining method's effectiveness across multiple tasks and scenarios, highlighting its versatility compared to other methods. This flexibility is a step toward developing a foundation model in the future, but we do not claim to have achieved that yet.

To avoid misunderstandings, we have revised the phrasing in the paper and removed any claims suggesting this is already a foundation model. We have also updated the title to reflect the scope and contributions of our work accurately.


\textbf{Q18: A figure showing which parts of the architecture are enabled for different test settings is requested.}

A18: Thanks for your suggestion! We have added more clear descriptions in the paper. As shown in \tabref{tab:setting_summary}, we load the weight of sparse encoder for indoor downstream testing and the weight of both encoder and BEV volume for outdoor downstream testing.


\textbf{Q19: In 4.1.2., It is not clear how the multi-frame rgbd is lifted into the voxel grid. Is the sparse backbone applied?}

A19: Thank you for pointing this out. Given a set of multiview RGB-D images, we back-project them into point clouds using known camera poses. This is a standard approach in computer vision and can be done with libraries like Open3D. Subsequent processes are the same as with scene point cloud inputs, where the point clouds are voxelized into sparse tensors. We have details on back-projection in Appendix~\ref{appx:rgbd_lift}.





